SparseVSR: Lightweight and Noise Robust Visual Speech Recognition

Recent advances in deep neural networks have achieved unprecedented success in visual speech recognition. However, there remains substantial disparity between current methods and their deployment in resource-constrained devices. In this work, we explore different magnitude-based pruning techniques to generate a lightweight model that achieves higher performance than its dense model equivalent, especially under the presence of visual noise. Our sparse models achieve state-of-the-art results at 10% sparsity on the LRS3 dataset and outperform the dense equivalent up to 70% sparsity. We evaluate our 50% sparse model on 7 different visual noise types and achieve an overall absolute improvement of more than 2% WER compared to the dense equivalent. Our results confirm that sparse networks are more resistant to noise than dense networks.

==> sections/related.tex <==
\section{Related work}
\label{sec:relatedwork}
\par{\noindent \bf{VSR:}}
Early works studied visual speech recognition using handcraft features and statistical approaches~\cite{fernandez2018survey}. 
In recent years, deep learning has revolutionised the field with the release of large-scale audiovisual datasets~\cite{son2017lip,afouras2018deep}. 
Work on lip-reading can roughly be divided into two groups. 
One trend is to use connectionist temporal classification (CTC)~\cite{shillingford2019large, afouras2020asr, ren2021learning}, where the model predicts labels per frame and then selects the optimal alignment between the frame-wise predictions and the output sequence. 
The second trend, try to process all the input sequences in an autoregressive manner, namely, attention-based sequence-to-sequence models (S2S)~\cite{afouras2018deep, ren2021learning}.
Recently, hybrid methods that combine both CTC and S2S were presented in~\cite{ma2022visual, ma2021end, ma2023auto}. Such methods incorporate a CNN frontend followed by a Conformer backend and a Transformer decoder. Inspired by this work, we present our VSR model in section \ref{sec:dense_model}. 


% \par{\noindent \bf{VSR:}} in recent years, there has been an increasing interest in decoding speech using only visual information, leading to lipreading models. Lipreading or VSR models are generally composed of an encoder that includes a pair of frontend and backend, and a decoder. The frontend is a CNN-based block that extracts visual features, e.g. a ResNet \cite{ren2021learning, ma2021end, ma2022visual}. Whereas the backend is based on RNNs (e.g. \cite{makino2019recurrent}), Transformers (e.g. \cite{serdyuk2021audio, ren2021learning, afouras2018deep}), or Conformers (e.g. \cite{ma2021end, ma2022visual}) that receive a sequence of relevant visual features and produces a latent representation at each time step. Finally, the decoder predicts the expected speech units, where there are two commonly used decoding strategies: i) connectionist temporal classification (CTC), ii) attention-based sequence-to-sequence (S2S). For example, authors in \cite{afouras2020asr, ren2021learning, afouras2018deep, shillingford2019large} use CTC, where the model predicts labels per frame and then selects the optimal alignment between the frame-wise predictions and the output sequence. Alternatively, authors in \cite{afouras2018deep, ren2021learning} use S2S models that process all of the input sequences before predicting the output sentence. Finally, there are also hybrid methods that combine the best of both benchmarks, shown in \cite{ma2021end, ma2022visual}. In this way, we find several works on continuous VSR in the English language due to the availability of large-scale audiovisual datasets, such as LRS2 and LRS3 \cite{afouras2018deep, shillingford2019large, makino2019recurrent, afouras2020asr, ren2021learning, ma2021end, serdyuk2021audio, shi2022learning, ma2022visual}. From those, very recently, Ma et al. \cite{ma2022visual} presented the current state-of-the-art on these datasets, which incorporate a CNN-based frontend followed by a Conformer backend and a Transformer decoder. The model is trained end-to-end using a combination of CTC/attention training. Inspired by this work, we present our baseline VSR model in section \ref{sec:dense_model}. 


%Thus, we base our VSR model on their work since their model achieves a 5\% and 8.2\% absolute improvement, in terms of the best Word Error Rate (WER) on LRS2 and LRS3, respectively, over the predecessor \cite{ma2021end}, under the same training data. 

% \par{\noindent \bf{Compression techniques:}} the development of ASR systems that fulfil different device requirements is challenging. Thus, several neural network compression techniques have been applied to speech recognition systems in general to overcome this issue, such as network pruning \cite{frankle2019lottery, chen2020lottery, ding2021audio}, knowledge distillation \cite{afouras2020asr, ren2021learning, li2018compression}, and parameter quantization \cite{sainath2020streaming}. For lipreading in particular, Afouras et al. \cite{afouras2020asr} proposed to distil knowledge from an ASR model trained on a large-scale audio-only corpus to a VSR model without requiring audio-visual annotated data. Similarly, Ren et al. \cite{ren2021learning} presented a distilling technique that uses bi-modal knowledge to close the inherent cross-modal gap. However, although both methods presented distilling techniques for VSR research their focus was not to reduce the computational and memory requirements of the VSR model but to propose a training strategy that takes advantage of audio resources to overcome state-of-the-art VSR models. Differently, in this work, \textbf{we propose to start from the state-of-the-art VSR model presented in \cite{ma2022visual} and train a noise-robust subnetwork without sacrificing performance}. Therefore, neural network pruning has evolved as the most common technique to achieve lower architectural complexity and higher performance under the same low-resource settings. From the counterpart ASR, very recent works have focused on pruning techniques \cite{yang2022omni, ding2021audio, lai2021parp}. For example, Yang et al. \cite{yang2022omni} proposed Omni-sparsity DNN, a supernet for ASR that maintain a single set of supernet model weights while generating sparse models for any target sparsity by applying pruning masks. The supernet finds, in a similar computational time than a single model, a family of sparse models, with 50\%-80\% sparsity, that perform 2\%-6.6\% better in WER. 
% In contrast, Ding et al. \cite{ding2021audio} investigate the possibility of using LTH to discover ASR models that are robust to acoustic noise, transferable and compatible with structured sparsity. In their experiments, they find small subnetworks for different architectures that match the full model at 80\% of sparsity. Moreover, when exposed to acoustic noise the subnetworks outperform the full models, showing noise robustness by inducing sparsity. On the other hand, Lai et al. \cite{lai2021parp} investigate the existence of sparse subnetworks in pre-trained self-supervised speech representation learning models that achieve better low-resource ASR results. They present Prune-Adjust-Re-Prune (PARP), which discovers and finetunes subnetworks, while only requiring a single downstream ASR finetuning run. They show that PARP discovers subnetworks  yields over 10\% WER reduction over the full model at high sparsities ($>$70\%).
% In this way, inspired by those works, we propose to investigate different pruning techniques to sparsify a VSR model and prove its robustness to different image noises.

\par{\noindent \bf{Compression:}} Model Compression is a process of developing deep learning models on edge devices that have low computing cost and memory without sacrificing  models' performance. It can be grouped in network pruning \cite{frankle2019lottery, han2015learning, renda2020comparing, frankle2021pruning}, knowledge distillation \cite{li2018compression,afouras2020asr, ren2021learning}, and parameter quantization \cite{gui2019model,sainath2020streaming}.
% Model compression has a long history in the machine learning literature and can be approximately grouped in network pruning \cite{frankle2019lottery, han2015learning, renda2020comparing, frankle2021pruning}, knowledge distillation \cite{li2018compression,afouras2020asr, ren2021learning}, and parameter quantization \cite{gui2019model,sainath2020streaming}.
Of more relevance to this work is network pruning, where the goal is to surpass/preserve the dense model performance while prune out some network weights, leading to a fast and lightweight model.
There are two main pruning techniques in the literature. 
The first is \textit{regularization and gradual pruning}, which prunes the model from the beginning and ends up with a pruned network~\cite{liu2022unreasonable}. For example, Liu et al. \cite{liu2022unreasonable} recently presented a random pruning method at initialization that achieves dense performance on CNN architectures. The second is \textit{retraining}, which prunes after the standard training ends \cite{frankle2019lottery}. 
The most common \textit{retraining} technique is \textit{fine-tuning}, which trains the pruned weights for a while at a fixed learning rate \cite{han2015learning}. In contrast, the authors of LTH \cite{frankle2019lottery} proposed \textit{weight rewinding}, which sets the unpruned weights back to its initial states and retrains using the original training schedule. 
They hypothesize that a network can reach full accuracy when trained in isolation from initialization. 
Follow-up work~\cite{ding2021audio} investigates the possibility of using LTH to discover ASR models that are robust to acoustic noise, transferable and compatible with structured sparsity. 
Apart from setting weights to the initial states, \cite{renda2020comparing} proposed \textit{learning rate rewinding} (LRR), which set the unpruned weights to their final values and retrains from there using the original learning rate schedule. Alternatively, Lai et al. \cite{lai2021parp} present PARP for self-supervised speech representation, where they discover subnetworks by allowing regrowth of their weights after pruning.
In this work, we extensively analyse various network pruning methods, setting the first benchmark in the VSR domain.

% \ie,~\cite{}; ii) \textit{retraining}, which prunes after the standard training process ends.~\cite{}
% Lai et al. \cite{lai2021parp} present PARP for self-supervised speech representation learning models. They discover and fine-tune subnetworks in a single downstream ASR run by allowing regrowth of their weights after pruning. Alternatively, the emergence of the LTH proposed a new strategy, known as \textit{weight rewinding} \cite{frankle2019lottery}. Differently from \textit{fine-tuning}, after pruning it rewinds the unpruned weights by setting their values back to its initial states or early states in training. They hypothesize that a network can reach full accuracy when trained in isolation from initialization \cite{frankle2019lottery}. Follow-up work~\cite{ding2021audio} investigates the possibility of using LTH to discover ASR models that are robust to acoustic noise, transferable and compatible with structured sparsity. In their experiments, they find small subnetworks for different architectures that match the full model at 80\% of sparsity. Moreover, when exposed to acoustic noise the subnetworks outperform the full models, showing noise robustness by inducing sparsity. On the other hand, subsequent research \cite{renda2020comparing} proposed \textit{learning rate rewinding} (LrRW), which instead of rewinding both learning rate and weights it only rewinds the learning rate schedule, i.e. it continues training the weights from the values at the end of the training. In this case, they hypothesize that retraining the model from the best possible initialization performs better. While literature on ASR and NLP investigated on the LTH \cite{yang2022omni, ding2021audio, chen2020lottery}, to the best of our knowledge there is no research for either weight and learning rate rewinding for VSR. 

% In the lipreading domain, knowledge distillation \cite{afouras2020asr, ren2021learning} was proposed to take advantage of the cross-model information to achieve better performance. Yet to the best of our knowledge, 
% similarly to other computer vision and speech recognition applications, the development of VSR systems that fulfil different device requirements is challenging. To deal with the aforementioned challenge, researchers have proposed several works on compression techniques, such as network pruning \cite{frankle2019lottery, han2015learning, renda2020comparing, frankle2021pruning}, knowledge distillation \cite{li2018compression}, and parameter quantization \cite{sainath2020streaming}. %, to decrease storage requirements and improve computational performance without compromising accuracy. 
% For lipreading, we find a few works on knowledge distillation \cite{afouras2020asr, ren2021learning}. However, their focus was not to reduce the computational and memory requirements of the VSR model, but to propose a training strategy that takes advantage of audio resources to overcome state-of-the-art VSR models. In contrast, other related tasks such as ASR or NLP, have recently applied pruning techniques for network compression \cite{yang2022omni, ding2021audio, lai2021parp, chen2020lottery}.
% There are two main pruning techniques in the literature: i) \textit{regularization and gradual pruning}, which end up with a pruned network at the end of the training~\cite{}; ii) \textit{retraining}, which prunes after the standard training process ends.~\cite{}
% However, training a subnetwork from start is difficult, leading to most of the approaches following a \textit{retraining} strategy. In this way, a dense network is trained to completion, then some of its structures are pruned following some heuristics and finally, the network is retrained for some time to recover the accuracy drop from pruning \cite{renda2020comparing}. Afterwards, the most common approach is to \textit{fine-tune} the subnetwork for extra $t$ epochs, i.e. you continue training with the final learning rate used for training \cite{han2015learning}. For example, 
% Lai et al. \cite{lai2021parp} present PARP for self-supervised speech representation learning models. They discover and fine-tune subnetworks in a single downstream ASR run by allowing regrowth of their weights after pruning. Alternatively, the emergence of the LTH proposed a new strategy, known as \textit{weight rewinding} \cite{frankle2019lottery}. Differently from \textit{fine-tuning}, after pruning it rewinds the unpruned weights by setting their values back to its initial states or early states in training. They hypothesize that a network can reach full accuracy when trained in isolation from initialization \cite{frankle2019lottery}. Follow-up work~\cite{ding2021audio} investigates the possibility of using LTH to discover ASR models that are robust to acoustic noise, transferable and compatible with structured sparsity. In their experiments, they find small subnetworks for different architectures that match the full model at 80\% of sparsity. Moreover, when exposed to acoustic noise the subnetworks outperform the full models, showing noise robustness by inducing sparsity. On the other hand, subsequent research \cite{renda2020comparing} proposed \textit{learning rate rewinding} (LrRW), which instead of rewinding both learning rate and weights it only rewinds the learning rate schedule, i.e. it continues training the weights from the values at the end of the training. In this case, they hypothesize that retraining the model from the best possible initialization performs better. While literature on ASR and NLP investigated on the LTH \cite{yang2022omni, ding2021audio, chen2020lottery}, to the best of our knowledge there is no research for either weight and learning rate rewinding for VSR.  



==> tables/Fig-absolute_difference_noise.tex <==
\begin{figure}[!tb]
  \centering
  \vspace{-0.2cm}
  \includegraphics[width=\columnwidth]{figures/abs_difference_50sp.pdf}
  \caption{Offset between dense and 50\% sparse BASE-L model using iterative LRR across noises and levels of corruption. \textit{Circle} represents seen noise types and \textit{Star} represents unseen ones. Positive values - improvement of the sparse model compared to the dense. Negative values - deterioration of it. }
  \label{fig:improvements_larg_model}
\end{figure}




==> tables/Fig-all-figures.tex <==
% \begin{table*}[tb]
% \begin{minipage}{.33\linewidth}
% \centering
% \includegraphics[width=1\textwidth]{figures/ablation_study_legend_right.pdf}
% \caption{WER of 20\%, 50\% and 80\% sparse BASE-S models evaluated on LRS3 when rewinded at different states $\theta_t$.}
% \label{fig:ablation_study}
% \end{minipage}
% \begin{minipage}{.33\linewidth}
% \centering
% \includegraphics[width=1\textwidth]{figures/seen_noises.pdf}
% \caption{Performance of dense and 50\% sparse BASE-L model using iterative LrRW on seen noise types.}
% \label{fig:seen_noises}
% \end{minipage}
% \begin{minipage}{.33\linewidth}
% \centering
% \includegraphics[width=1\textwidth]{figures/unseen_noises.pdf}
% \caption{Performance of dense and 50\% sparse BASE-L model using iterative LrRW on seen noise types.}
% \label{fig:unseen_noises}
% \end{minipage}
% \end{table*}

\begin{figure*}[tb]
\centering %
\floatsetup{floatrowsep=qquad}
\begin{floatrow}[3]%
\ffigbox[]{\caption{WER of 20\%, 50\% and 80\% sparse BASE-S models evaluated on LRS3 when rewinded at different states $\theta_t$.}\label{fig:ablation_study}}{\includegraphics[width=1\columnwidth, trim=0.2cm 0cm 0.2cm 0.2cm, clip]{figures/ablation_study_legend_right.pdf}}
\vspace{-.2cm}
\ffigbox[]{\caption{Performance of dense (d) and 50\% sparse (sp) BASE-L models on LRS3 test set corrupted by BW, GB, MB and P noises at different levels (level 0 means clean data). The sparse model is compressed by iterative pruning LrWD}\label{fig:seen_noises}}{\includegraphics[width=\columnwidth, trim=0.2cm 0cm 0.2cm 0.2cm, clip, clip]{figures/seen_noise.pdf}}
\vspace{-.2cm}
\ffigbox[]{\caption{Performance of dense (d) and 50\% sparse (sp) BASE-L models on LRS3 test set corrupted by GN, VC and C noises at different levels (level 0 means clean data). The sparse model is compressed by iterative pruning LrWD.}\label{fig:unseen_noises}}{\includegraphics[width=\columnwidth, trim=0.2cm 0cm 0.2cm 0.2cm, clip, clip]{figures/unseen_noise.pdf}}
\vspace{-.2cm}
\end{floatrow}
\end{figure*}

==> tables/Fig-dense_50_sparse_noises.tex <==
\begin{figure}[!tb]
  \centering
  \vspace{-0.2cm}
  \includegraphics[width=\columnwidth]{figures/dense_50_sparse_noises.pdf}
  \caption{Performance of dense and 50\% sparse BASE-L model using iterative LRR on LRS3 corrupted test set. }
  \label{fig:dense_50_sparse_noises}
\end{figure}

==> tables/Tab-Absolute_diff_all_sparsities.tex <==
% \begin{table}[]
% \begin{tabular}{lccccccc}
% \textbf{Sp} & \textbf{BW} & \textbf{GB} & \textbf{MB} & \textbf{P} & \textbf{C} & \textbf{GN} & \textbf{VC} \\
% 0           & 4.87        & 3.82        & 4.75        & 31.2       & 27.4       & 81.4        & 77.1        \\
% 10\%        & 4.63        & 3.03        & 4.37        & 31.0       & 27.6       & 79.6        & 77.9        \\
% 20\%        & 4.06        & 3.02        & 3.74        & 29.5       & 26.3       & 75.3        & 77.3        \\
% 30\%        & 4.00        & 3.36        & 3.78        & 29.2       & 26.8       & 72.8        & 77.4        \\
% 40\%        & 3.59        & 2.99        & 2.91        & 28.0       & 27.9       & 67.5        & 76.8        \\
% 50\%        & 3.86        & 3.53        & 3.63        & 28.9       & 29.0       & 67.3        & 78.1        \\
% 60\%        & 3.77        & 3.76        & 3.52        & 28.7       & 28.8       & 73.4        & 77.6        \\
% 70\%        & 4.49        & 3.59        & 3.62        & 29.2       & 29.2       & 77.7        & 77.5        \\
% 80\%        & 5.66        & 3.87        & 4.03        & 30.2       & 30.7       & 75.1        & 75.3        \\
% 90\%        & 7.51        & 5.6         & 5.17        & 33.1       & 33.6       & 72.5        & 70.6       
% \end{tabular}
% \end{table}


\begin{table}[!htb]
\caption{Absolute difference between level 10 of corruption and clean data for dense and sparse BASE-L models.}
%\vspace{-.2cm}
\label{tab:level10clean}
\setlength{\tabcolsep}{0.8pt}
\centering
\begin{threeparttable}
\begin{tabular}{l|cccccccccc}
\toprule
\textbf{N/Sp} & \textbf{0} & \textbf{10\%} & \textbf{20\%} & \textbf{30\%} & \textbf{40\%} & \textbf{50\%} & \textbf{60\%} & \textbf{70\%} & \textbf{80\%} & \textbf{90\%} \\ \midrule
\textbf{BW}       & 4.87       & 4.63          & 4.06          & 4.00             & 3.59          & 3.86          & 3.77          & 4.49          & 5.66          & 7.51          \\
\textbf{GB}       & 3.82       & 3.03          & 3.02          & 3.36          & 2.99          & 3.53          & 3.76          & 3.59          & 3.87          & 5.60           \\
\textbf{MB}       & 4.75       & 4.37          & 3.74          & 3.78          & 2.91          & 3.63          & 3.52          & 3.62          & 4.03          & 5.17          \\
\textbf{P}        & 31.1       & 30.9          & 29.4          & 29.1          & 28.0          & 28.9          & 28.6          & 29.1          & 30.1          & 33.0          \\
\textbf{C}        & 27.4       & 27.5          & 26.3          & 26.7          & 27.8          & 28.9          & 28.7          & 29.2          & 30.6          & 33.5          \\
\textbf{GN}       & 81.3       & 79.5          & 75.2          & 72.7          & 67.4          & 67.3          & 73.4          & 77.6          & 75.1          & 72.5         \\
\textbf{VC}       & 77.1       & 77.8          & 77.2          & 77.4          & 76.7          & 78.0          & 77.5          & 77.4          & 75.3          & 70.6         \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table}



